Exploring Magnitude Preservation and Rotation Modulation in Diffusion Transformers

Denoising diffusion models exhibit remarkable generative capabilities, but remain challenging to train due to their inherent stochasticity, where high-variance gradient estimates lead to slow convergence. Previous works have shown that magnitude preservation helps with stabilizing training in the U-net architecture. This work explores whether this effect extends to the Diffusion Transformer (DiT) architecture. As such, we propose a magnitude-preserving design that stabilizes training without normalization layers. Motivated by the goal of maintaining activation magnitudes, we additionally introduce rotation modulation, which is a novel conditioning method using learned rotations instead of traditional scaling or shifting. Through empirical evaluations and ablation studies on small-scale models, we show that magnitude-preserving strategies significantly improve performance, notably reducing FID scores by $\sim$12.8%. Further, we show that rotation modulation combined with scaling is competitive with AdaLN, while requiring $\sim$5.4% fewer parameters. This work provides insights into conditioning strategies and magnitude control. We will publicly release the implementation of our method.

==> data/convergence-b4.tex <==
\defdata{e_b_4-guid---steps-is}{
(50000,  20.8534)
(100000, 29.8199)
(150000, 37.9015)
(200000, 44.4367)
(250000, 48.6114)
(300000, 53.9366)
(350000, 60.2587)
(400000, 65.6078)
}
\defdata{e_b_4-guid---steps-is-argmax}{8}
\defdata{e_b_4-guid---steps-is-max}{}

\defdata{e_b_4-guid---steps-fid10k}{
(50000,  57.5303)
(100000, 47.1518)
(150000, 39.2219)
(200000, 36.1130)
(250000, 33.4135)
(300000, 32.4520)
(350000, 29.0872)
(400000, 28.3903)
}
\defdata{e_b_4-guid---steps-fid10k-argmin}{8}
\defdata{e_b_4-guid---steps-fid10k-min}{}

\defdata{e_b_4-guid---steps-sfid10k}{
(50000,  34.7040)
(100000, 33.0303)
(150000, 31.8135)
(200000, 28.571)
(250000, 28.1131)
(300000, 29.9558)
(350000, 28.1436)
(400000, 29.2748)
}
\defdata{e_b_4-guid---steps-sfid10k-argmin}{8}
\defdata{e_b_4-guid---steps-sfid10k-min}{}

\defdata{e_b_4-guid---steps-precision}{
(50000,  0.2874)
(100000, 0.3929)
(150000, 0.4602)
(200000, 0.5097)
(250000, 0.5483)
(300000, 0.5574)
(350000, 0.6021)
(400000, 0.6047)
}
\defdata{e_b_4-guid---steps-precision-argmax}{8}
\defdata{e_b_4-guid---steps-precision-max}{}

\defdata{e_b_4-guid---steps-recall}{
(50000,  0.2219)
(100000, 0.2535)
(150000, 0.2842)
(200000, 0.2777)
(250000, 0.3025)
(300000, 0.2939)
(350000, 0.3086)
(400000, 0.3002)
}
\defdata{e_b_4-guid---steps-recall-argmax}{8}
\defdata{e_b_4-guid---steps-recall-max}{}
